Bayesian Action Decoder for Deep Multi-Agent Reinforcement Learning

When observing the actions of others, humans make inferences about why they acted as they did, and what this implies about the world; humans also use the fact that their actions will be interpreted in this manner, allowing them to act informatively and thereby communicate efficiently with others. Although learning algorithms have recently achieved superhuman performance in a number of two-player, zero-sum games, scalable multi-agent reinforcement learning algorithms that can discover effective strategies and conventions in complex, partially observable settings have proven elusive. We present the Bayesian action decoder (BAD), a new multi-agent learning method that uses an approximate Bayesian update to obtain a public belief that conditions on the actions taken by all agents in the environment. BAD introduces a new Markov decision process, the public belief MDP, in which the action space consists of all deterministic partial policies, and exploits the fact that an agent acting only on this public belief state can still learn to use its private information if the action space is augmented to be over all partial policies mapping private information into environment actions. The Bayesian update is closely related to the theory of mind reasoning that humans carry out when observing others' actions. We first validate BAD on a proof-of-principle two-step matrix game, where it outperforms policy gradient methods; we then evaluate BAD on the challenging, cooperative partial-information card game Hanabi, where, in the two-player setting, it surpasses all previously published learning and hand-coded approaches, establishing a new state of the art.

==> core/5_experiments.tex <==


\section{Experiments and Results}
\label{sec:experiments}


\subsection{Matrix Game}
We first present proof-of-principle results for a two-player, two-step partially observable matrix-like game (Figure~\ref{fig:tiny_hanabi}). The state consists of 2 random bits (the cards for Player 1 and 2) and the action space consists of 3 discrete actions. 
Each player observes its own card, with Player 2 also observing Player 1's action before acting, which in principle allows Player 1 to encode information about its card with its action.
The reward is specified by a payoff tensor, $r = \mathrm{Payoff}[\text{card}^1][\text{card}^2][u^1][u^2]$, where $\text{card}^a$ and $u^a$ are the card and action of the two players, respectively. The payout tensor is structured such that the optimal reward can only be achieved if the two players establish a convention, in particular if Player 1 chooses informative actions that can be decoded by Player 2.

As shown in Figure~\ref{fig:matrix_game_result}, BAD clearly outperforms the baseline policy-gradient method on the toy matrix game. In this small, exact setting, it is also possible to estimate counterfactual (CF) policy gradients that reinforce not only the action taken, but also these counterfactual actions. This can be achieved by replacing $\log \pi^a( u^a_t | \tau^a) $ with $\log P(\pidet  |  \pubB_t,  f^\text{pub})$ in the estimation of the policy gradient. \sw{cite EPG?} However, the additional improvement in performance from using CF gradients is minor compared to the initial performance gain from  using a counterfactual belief state. 
%
Code %for the matrix game with a proof-of-principle implementation of BAD 
is available at \url{https://bit.ly/2P3YOyd}.%  in the Supplemental Material. %\url{bit.ly/2PYvGow}
%[link available for final copy].


  \begin{figure}[t!]
 	\centering
	
	\begin{subfigure}[b]{0.95\linewidth}
		\includegraphics[width=\linewidth]{figs/tinyhanabi_learning}
 	\end{subfigure}
	 	\caption{BAD, both with and without counterfactual (CF) gradients, outperforms vanilla policy gradient on the matrix-like game. Each line is the mean over 1000 games, and the shade indicates the standard error of the mean (s.e.m.).}
 	\label{fig:matrix_game_result}
 \end{figure}

 
\subsection{Hanabi}
Here we briefly describe the rules of Hanabi. 
Let $N_h$ the number of cards in a hand. In the standard game of Hanabi, $N_h=5$ for $A=$ 2 or 3 and $N_h=4$ for $A=$ 4 or 5 players. For generality, we consider that for each colour there are three cards  with $\text{rank} = 1$, one with $\text{rank} =N_\text{rank}$, and two each with $\text{rank} =2,\ldots,(N_\text{rank}-1)$, i.e., $2N_\text{rank}$ cards per colour for a total of $N_\text{deck}=2N_\text{color}N_\text{rank}$ cards in the deck. In the standard game of Hanabi, $N_\text{color}=N_\text{rank}=5$ for a total of $N_\text{deck}=50$. While this is a modestly large number of cards, even for 2 players it leads to $6.2 \times 10^{13}$ possible joint hands at the beginning of the game. 

\subsection{Observations and Actions}
Each player observes the hands of all other players, but not their own. The action space consists of $N_h \times 2$ options for discarding and playing cards, and $N_\text{color} + N_\text{rank}$ options per teammate for hinting colours and ranks. Hints reveal all cards of a specific rank or colour to one of the teammates, e.g., ``Player 2's card 3 and 5 are red''. Hinting for colours and ranks not present in the teammate's hand (``empty hints'') is not allowed.

Each hint costs one hint token. The game starts with eight hint tokens, which can be recovered by discarding cards. After a player has played or discarded a card, they draw a new card from the deck. When a player picks up the last card, everyone (including that player) gets to take one more action before the game terminates.
Legal gameplay consists of building $N_\text{color}$ fireworks, which are piles of ascending numbers, starting at one, for each colour. When the $N_\text{rank}$-th card has been added to a pile the firework is complete and the team obtains another hint token (unless they already have eight).
Each time an agent plays  an illegal card the players lose a life token; after three mistakes the game also terminates. 
Players receive one point after playing any playable card, with a perfect score being $N_\text{color}N_\text{rank}$.

The number of hint and life tokens at any time are observed by all players, as are the played and discarded cards, the last action of the acting player, and any hints provided.

 
\subsection{Beliefs in Hanabi}
\label{sec:beliefs_in_hanabi}
The basic belief calculation in Hanabi is straightforward: $f_t^\text{pub}$ consists of a vector of \emph{candidates} $C$ containing counts for all remaining cards, and a \emph{hint mask} $\text{HM}$, an $AN_h\times (N_\text{color}N_\text{rank}+1)$ binary matrix that is one if in a given \emph{slot} the player could be holding a specific card according to the hints so far, and $0$ otherwise; the additional 1 accounts for the possibility that the card may not exist in the final round of play. Slots correspond to the features of the private state space $\fei$, for example the third card of the second player. Hints contain both positive and negative information: for example, the statement ``the second and fourth cards are red'' also implies that all other cards are not red.

The basic belief $B^0$ can be calculated as
\begin{equation}
B^0(\fei)= P(\fei | f^\text{pub} ) \propto C(f) \times \text{HM}(\fei).
\end{equation}
 We call this the \emph{V0 belief}, in which the belief for each card depends only on the publicly available information for that card. In our experiments, we focus on baseline agents that receive this basic belief, rather than the raw hints, as public observation inputs; while the problem of simply remembering all hints and their most immediate implication for card counts is potentially challenging for humans in recreational play, we are here more interested in the problem of forming effective conventions for high-level play.
  
As noted above, this basic belief misses an important interaction between the hints for different slots.  
We can calculate an approximate version of the self-consistent beliefs that avoids the potentially expensive and noisy sampling step in \eqref{eq:B_kp1}:
\begin{equation}
B^{k+1}(\fei) \propto \Bigg( C(f)  - \sum_{j \neq i} B^{k}(\fej) \Bigg)   \times \text{HM}(\fei).
\end{equation}
A derivation is in the Supplemental Material. This sampling is distinct from the sampling required to compute the marginal likelihood in \eqref{eqn:bad-sampling}.
 
We call the resulting belief at convergence (or after a maximum number of iterations) the \emph{V1 belief}. It does not condition on the Bayesian probabilities but considers interactions between hints for different cards. In essence, at each iteration the belief for a given slot is updated by reducing the candidate count by the number of cards believed to be held across all other slots.
 
By running the same algorithm but including ${\cal L}$, we obtain the Bayesian beliefs $\text{BB}$ that lie at the core of BAD:
\begin{align}
	\text{BB}^0 (\fei) & \propto C(f)  \times \text{HM}(\fei) \times {\cal L}(\fei),  \\
\text{BB}^{k+1}(\fei) &\propto \Bigg( C(f)   - \sum_{j \neq i} B^{k}(\fej) \Bigg) \notag \\ &\qquad \times  \text{HM}(\fei) \times {\cal L}(\fei).
\end{align}
In practice, to ensure stability, the final \emph{V2 belief} that we use is an interpolation between the Bayesian belief and the V1 belief: $\text{V2} = (1 - \alpha) \text{BB} +  \alpha \text{V1}$ with $\alpha=0.01$ (we found $\alpha=0.1$ to also work). 
 
 
  \begin{figure*}[t!]
 	\centering
	
 	\begin{subfigure}[b]{0.32\linewidth}
		\includegraphics[width=\linewidth]{figs/fullgame_learning}
		\caption{}
 	\end{subfigure}
	\begin{subfigure}[b]{0.32\linewidth}
  		\includegraphics[width=\linewidth]{figs/fullgame_score_histogram}
		\caption{}
 	\end{subfigure}
	\begin{subfigure}[b]{0.32\linewidth}
  		\includegraphics[width=\linewidth]{figs/fullgame_beliefs}
		\caption{}
 	\end{subfigure}
	 	\caption{a) Hanabi training curves for BAD and the V0 and V1 baseline methods using LSTMs rather than the Bayesian belief. Thick lines indicate the final evaluated agent for each agent type, with the dots showing the final test score. Error bars (standard error of the mean, s.e.m.) are smaller than the dots. Upward kinks in the curves are generally due to agents `evolving' in PBT by copying its weights and hyperparameters (plus perturbations) from a superior agent.
 	b) Distribution of game scores for BAD on Hanabi under testing conditions. BAD achieves a perfect score in almost $60\%$ of the games. The dashed line shows the proportion of perfect games reported for FireFlower, the best known hard-coded bot for two-player Hanabi. c) Per-card cross entropy with the true hand for different belief mechanisms in Hanabi during BAD play. V0 is the basic belief based on hints and card counts, V1 is the self-consistent belief, and V2 is the BAD belief which also includes the Bayesian update. The BAD agent conveys around $40\%$ of the information via conventions, rather than grounded information.}
 	\label{fig:full_game}
 \end{figure*}

 
\subsection{Architecture Details for Baselines and Method}
Advantage actor-critic agents were trained using the Importance-Weighted Actor-Learner Architecture \cite{Espeholt2018}, in particular the multi-agent implementation described by \citeauthor{Jaderberg2018} (\citeyear{Jaderberg2019}). In this framework, \emph{actors} continually generate trajectories of experience (sequences of states, actions, and rewards) by having agents (self-)playing the game, which are then used by \emph{learners} to perform batched gradient updates (batch size was 32 for all agents). Because the policy used to generate the trajectory can be several gradient updates behind the policy at the time of the gradient update, V-trace \sw{cite?} was applied to correct for the off-policy trajectories. The length of the trajectories, or rollouts, was 65, the maximum length of a winning game.

In the V0-LSTM and V1-LSTM agents, all observations were first processed by an MLP with a single 256-unit hidden layer and ReLU activations, then fed into a two-layer LSTM with 256 units in each layer. The policy $\pi$ was a softmax readout of the LSTM output. The baseline network was an MLP with a single 256-unit hidden layer and ReLU activations, which then projected linearly to a single value. Since the baseline network is only used to compute gradient updates, we followed \citeauthor{Foerster2017} (\citeyear{Foerster2017}) in feeding each agent's own hand (i.e., the other agent's private observation) into the baseline by concatenating it with the LSTM output; thus we make the common assumption of centralised training and decentralised execution. We note that the V0 and V1-LSTM agents differed \emph{only} in their public belief inputs.

The BAD agent consisted of an MLP with two 384-unit hidden layers and ReLU activations that processed all observations, followed by a linear softmax policy readout. To compute the baseline, we used the same MLP as the policy but included the agent's own hand in the input (this input was present but zeroed out for the computation of the policy).

For all agents, illegal actions (such as hint for a red card when there are no red cards) were masked out by setting the corresponding policy logits to a large negative value before sampling an action. In particular, for the non-acting agent at each turn the only allowed action was the \emph{no-action}.

Descriptions of the hyperparameters and additional training details are given in the Supplemental Material.


\subsection{Results on Hanabi}

The BAD agent achieves a new state-of-the-art mean performance of \finalperformance{} points on two-player Hanabi. Figure~\ref{fig:full_game}a shows training curves and test performance for BAD and two LSTM-based baseline methods, as well as the performance of FireFlower (\url{https://github.com/lightvector/fireflower}), the best known hand-coded bot for two-player Hanabi. For the LSTM agents, test performance was obtained by using the greedy version of the trained policy, resulting in slightly higher scores than during training. To select the agent, we first performed a sweep over all agents for 10,000 games, then carried out a final test run of 100,000 games on the best agent from the sweep, since taking the maximum of a sweep introduces bias in the score. We used a similar procedure for the BAD agent but with additional hyperparameters, also varying the V1 mix-in factor, and number of sampled hands.

The results for other learning methods from the literature perform well below the range of the $y$-axis (far below 20 points) and are omitted for readability. We note that, under a strict interpretation of the rules of Hanabi, games in which all three error tokens are exhausted should be awarded a score of zero. Under these rules the same BAD agent achieves $23.917 \pm 0.009$ s.e.m., still better than both hand-coded bots. Note that SmartBot only reported results for when all points are counted, while FireFlower achieves a lower score of 22.56 $\pm$ 0.00 on average under this accounting. This is true even though our agents were not trained under these conditions.

 \begin{table}[t!]
	\begin{center}
		\resizebox{\linewidth}{!}{
			\begin{tabular}{c ccc}
				\toprule
				
				\multirow{2}{*}{Agent} 
				& \multirow{2}{*}{Learning steps} 
				& \multirow{2}{*}{Mean $\pm$ s.e.m.}
				& \multirow{2}{*}{Prop. perfect}
				\\
				&  &  &  \\

				\midrule
				SmartBot & - & 23.09 & 29.52\% \\
				FireFlower & - & 23.37 $\pm$ 0.0002 & 52.6\% \\
				V0-LSTM & 20.2B  & 23.622 $\pm$ 0.005 & 36.5\% \\
				V1-LSTM & 21.1B  & 23.919 $\pm$ 0.004 & 47.5\% \\
				% BAD & 9.6B & \textbf{\finalperformance{} $\pm$ 0.004} & \textbf{53.2\%} \\
				BAD & \finalsteps B & \textbf{\finalperformance $\pm$ 0.004} & \textbf{\finalperfectgames\%} \\
				\bottomrule

			\end{tabular}
		}
	\end{center}
	\caption{Test scores on 100K games. The LSTM agents were tested with a greedy version of the trained policy, while the final BAD agent was evaluated with V1 mix-in $\alpha=0.01$, 20K sampled hands, and inverse softmax temperature 100.0. The FireFlower bot was evaluated over 25K games.}
	\label{tbl:scores}
	
\end{table}

While not all of the gameplay BAD learns is easy to follow, some conventions can be understood simply from inspecting the game. Printouts of 100 random games can be found at \url{https://bit.ly/2zeEShh}. %in the Supplemental Material. %\url{bit.ly/2wGYREP}. 
One convention stands out:  Hinting for `red' or `yellow' indicates that the newest card of the other player is playable. We found that in over $80\%$ of cases when an agent hints `red' or `yellow',  the next action of the other agent is to play the newest card.
This convention is powerful: typically agents know the least about the newest card, so by hinting `red' or `yellow', agents can use a single hint to tell the other agent that the card is playable. Indeed, the use of two colours to indicate ``play newest card'' was present all of the highest performing agents we studied. Hinting `white' and `blue' are followed by a discard of the newest card in over $25\%$ of cases. We also found that the agent sometimes attempts to play cards that are not playable in order to convey information to their team mate. 
In general, unlike human players, agents predominantly play and discard the last card. 


Figure~\ref{fig:full_game}c shows the quality of the different beliefs. While the iterated belief update leads to a reduction in cross entropy compared to the basic belief, a much greater reduction in cross entropy is obtained using counterfactual beliefs. This clearly demonstrates the importance of learning conventions for successful gameplay in Hanabi: roughly $40\%$ of the information is obtained through conventions rather than through the grounded information and card counting. 





==> core/6_results.tex <==


%\section{Results}
%\begin{figure}[t!]
% 	\centering
%	
% 	\begin{subfigure}[b]{1\linewidth}
%		\includegraphics[width=\linewidth]{figs/tinyhanabi_matrix}
%		\caption{}
% 	\end{subfigure}
%	\begin{subfigure}[b]{1\linewidth}
%  		\includegraphics[width=\linewidth]{figs/tinyhanabi_learning}
%		\caption{}
% 	\end{subfigure}
%	
% 	\caption{Tiny Hanabi. (a) Payoff matrix for Tiny Hanabi. The first two dimensions correspond to the card held by each player, the last two dimensions to the action chosen by each player. (b) BAD, both with and without gradients, outperforms vanilla policy gradient on Tiny Hanabi over 1000 games. For each line the shade indicates SEM.}
% 	\label{fig:tiny_hanabi}
% \end{figure}



		
		%m5v5
		%Mean Avg Win % (std %)
		%IAC-V: 62.65 ( 4.41, 1.61 )
		%IAC-Q: 58.37 ( 8.22, 3.00 )
		%central-V: 66.66 ( 12.90, 4.71 )
		%central-QV: 71.40 ( 24.25, 8.86 )
		%COMA: 81.01 ( 12.80, 4.68 )
		
		
		%m3v3
		%Mean Avg Win % (std %)
		%IAC-V: 47.11 ( 9.83, 3.37 )
		%IAC-Q: 55.65 ( 17.70, 6.07 )
		%central-V: 83.06 ( 10.16, 3.48 )
		%central-QV: 82.53 ( 13.26, 4.55 )
		%COMA: 87.40 ( 7.77, 2.66 )
		
		
		%w5v5
		%Mean Avg Win % (std %)
		%IAC-V: 17.71 ( 13.08, 4.70 )
		%IAC-Q: 57.39 ( 15.09, 5.42 )
		%central-V: 65.00 ( 7.46, 2.68 )
		%central-QV: 75.63 ( 4.01, 1.44 )
		%COMA: 82.05 ( 7.43, 2.67 )
		
		

